Differentially Private Representation Learning via Image Captioning

Differentially private (DP) machine learning is considered the gold-standard solution for training a model from sensitive data while still preserving privacy. However, a major barrier to achieving this ideal is its sub-optimal privacy-accuracy trade-off, which is particularly visible in DP representation learning. Specifically, it has been shown that under modest privacy budgets, most models learn representations that are not significantly better than hand-crafted features. In this work, we show that effective DP representation learning can be done via image captioning and scaling up to internet-scale multimodal datasets. Through a series of engineering tricks, we successfully train a DP image captioner (DP-Cap) on a 233M subset of LAION-2B from scratch using a reasonable amount of computation, and obtaining unprecedented high-quality image features that can be used in a variety of downstream vision and vision-language tasks. For example, under a privacy budget of $\varepsilon=8$ for the LAION dataset, a linear classifier trained on top of learned DP-Cap features attains $65.8\%$ accuracy on ImageNet-1K, considerably improving the previous SOTA of $56.5\%$.

==> Untitled/1-intro.tex <==
\begin{figure*}[t!]
     \centering
     \includegraphics[width=0.99\textwidth]{figs/DP-MULTIMODAL.pdf}
     \vspace{-0.05in}
    \caption{(a) Few-shot ImageNet-1K linear probe accuracy comparison between DP-Cap (ours) and ViP~\citep{yu2023vip} (previous SOTA). DP-Cap learns better image representations using the same training data and privacy budget, and considerably surpasses synthetic initialization (\emph{syn}). \revisioncolor{The privacy budget $\varepsilon$ is for the LAION dataset, and the linear classifiers are trained without DP.} (b) Compositional understanding evaluation on the ARO benchmark~\citep{yuksekgonul2022and}. DP-Cap performance is close to non-private Cap and outperforms non-private CLIP. (c) Captions generated by DP-Cap on images from the MS-COCO 2017~\citep{lin2015microsoft} test set.}
    \label{fig:1}
    \vspace{-0.1in}
\end{figure*}

\section{Introduction}
\label{sec:introduction}

Differentially private (DP; \citet{dwork2006calibrating}) model training is an effective strategy for privacy-preserving ML on sensitive data. For most optimization-based learning algorithms, DP-SGD~\citep{song2013stochastic, abadi2016deep} can be readily applied to obtain models with rigorous DP guarantee. Regrettably, DP training has also been marred by a sub-optimal privacy-utility trade-off, with model utility severely lagging behind their non-private counterpart~\citep{jayaraman2019evaluating, tramer2020differentially, kurakin2022toward}. At the core of this unfavorable trade-off is the \emph{difficulty of DP representation learning}. \citet{tramer2020differentially} showed that when DP training from scratch under a low-to-moderate privacy budget, most models do not learn useful representations, with the quality of learned representations worse than even handcrafted features. 
These observations naturally lead to the research question: \emph{``How does one learn useful representations with DP training?''}

One plausible reason for the failure of prior attempts at DP representation learning is the lack of training data. Indeed, DP limits the information content of each training sample via the privacy budget $\varepsilon$, inducing a privacy-accuracy-sample size tradeoff; thus a substantially larger training dataset is required to extract the same amount of information to train the model. As the vast majority of prior work only utilize small to moderate scale classification datasets such as CIFAR-10~\citep{krizhevsky2009learning} and ImageNet~\citep{deng2009imagenet}, the amount of training data is simply insufficient for learning high-quality representations under DP~\citep{tramer2020differentially}.
\citet{yu2023vip} made partial progress towards this through \emph{self-supervised learning} (SSL) on \emph{internet-scale data}. By training a masked autoencoder (MAE; \citet{he2022masked}) using DP-SGD on a 233M subset of the LAION-2B dataset~\citep{Schuhmann2022LAION5BAO}, the model learned image representations that are on-par with non-private AlexNet~\citep{krizhevsky2012imagenet} trained on ImageNet---the first deep learning model to outperform handcrafted features and a major cornerstone for representation learning.
However, the MAE objective also promotes the model to learn extraneous details in the image that may not be helpful for obtaining generalizable representations, severely limiting the potential of this approach for DP.

We adopt a different approach of DP training via image captioning on internet-scale multimodal datasets. The reason is twofold: \textbf{1.} Text caption provides a concise summary of the training image and serves as better supervision compared to image-only SSL~\citep{tschannen2023image}. Under the constraint on information content from DP, we hypothesize that it provides substantially more efficient information extraction under DP training.
\textbf{2.} Image captioning is well-aligned with the prerequisites of DP-SGD such as having an instance-separable loss.
We apply this method on a 233M subset of LAION-2B to train a DP image captioning model (DP-Cap), whose learned representations surpass previous SOTA---ViP~\citep{yu2023vip}---by a large margin. As depicted in Figure~\ref{fig:1}(a), our model trained with a privacy budget of $\varepsilon=8$ shows substantial improvements on
downstream tasks compared to ViP, both trained on the same dataset. To achieve this, we also made crucial improvements to the efficiency of the DP training pipeline, \textbf{reducing the compute cost by close to $\mathbf{5\times}$} on the largest model.

The image representations learned by DP-Cap also exhibit strong performance for multimodal tasks that require alignment of image and text features,
the first occurrence for models trained from scratch with DP; see Figure~\ref{fig:1}(b).
As a qualitative evaluation, we also use the trained DP-Cap model to caption several images from the MS-COCO 2017~\citep{lin2015microsoft} test set in Figure~\ref{fig:1}(c) and Appendix~\ref{subsec:appendix-image-caption}. The resulting captions are grammatically correct and semantically coherent, while (close to) accurately describing contents of the image; this is interesting because our model has only been exposed to language supervision from LAION, which are far from being flawless.
Our results suggest that DP training on internet-scale multimodal datasets can be a viable approach for obtaining high-utility learned representations.




























==> Untitled/2-prelim.tex <==
\section{Background and Related Work}
\label{sec:background}












\textbf{Vision-language pre-training.} Many modern ML datasets such as Conceptual Captions~\citep{changpinyo2021conceptual}, LAION~\citep{schuhmann2021laion} and DataComp~\citep{gadre2023datacomp} consist of aligned image-text pairs where the image and text contain roughly similar semantic information. One can leverage the aligned nature of the training data to pre-train \emph{vision-language models} (VLMs) that connect the two modalities, whose representations perform more general multi-modal tasks. Contrastive learning-based techniques such as CLIP~\citep{radford2021learning} and BLIP~\citep{li2022blip} are also applicable for pre-training VLMs.
Doing so not only learns high-quality image and text representations but also introduces new multi-modal capabilities such as cross-modal retrieval and zero-shot prediction~\citep{radford2021learning}.
Recent work by \cite{tschannen2023image} shows an image captioning approach (predicting text captions from images) is a viable alternative to contrastive learning and can lead to models with robust performance.


\textbf{Differential privacy \citep{dwork2006calibrating}.} In the following, we denote by $\calM$ a randomized learning algorithm, which takes a dataset $\mathcal{D}$ containing $N$ samples and produces a machine learning model $\bm{\theta}$ through the process $\calM(\mathcal{D})$.
A randomized mechanism $\calM$ is $(\varepsilon, \delta)$-DP if, for any two adjacent datasets $\mathcal{D}$ and $\mathcal{D}^{\prime}$ differing by a single sample, and for any subset $\mathcal{O}\subset \mathbf{Im}(\calM)$:
\begin{equation}\label{eq:def-dp}
    \mathbf{P}[\calM(\mathcal{D}) \in \mathcal{O}] \leq \mathbf{P}[\calM(\mathcal{D}^{\prime}) \in \mathcal{O}] \exp( \varepsilon) + \delta.
\end{equation}
We adopt the leave-one-out notion of adjacency in this work, \emph{i.e.}, $\mathcal{D} = \mathcal{D}^{\prime} \cup \{\mathbf{x}\}$ for some sample $\mathbf{x}$ or vice versa. DP bounds the extent to which any potential adversary can infer information about the dataset $\mathcal{D}$ after observing the algorithm's output.
In the context of ML, this implies that if we obtain the model $\bm{\theta}$ through a DP training algorithm $\calM$ then its training data is provably difficult to recover or infer~\citep{balle2022reconstructing, guo2022bounding,guo2023analyzing}. 




\textbf{DP-SGD}~\citep{song2013stochastic, abadi2016deep} is predominant differentially private algorithm for training deep neural networks (DNNs).
At each gradient step $k$, a batch $\mathcal{B}_k$ is sampled where each example from the training data is chosen randomly with probability $q=B/N$, where $B$ represents the average batch size. 
For $C >0$, define the clipping function for any $X \in \mathbb{R}^d$ by $\mathrm{clip}_C(X) = C\cdot X/\Vert X \Vert$ if $\Vert X \Vert \geq C$ and $\mathrm{clip}_C(X) = X$ otherwise.
Given model parameters $\bm{\theta}_k$, DP-SGD defines the update
$\bm{\theta}_{k+1} = \bm{\theta}_k -\eta_k \widetilde{\mathbf{g}}_k$ where $\eta_k$ is the step size and $\widetilde{\mathbf{g}}_k$ is given by:
\begin{equation}
\label{eq:DP_SGD}
{\small 
\widetilde{\mathbf{g}}_k := \frac{1}{B} \left[ \sum_{i \in \mathcal{B}_k} \text{clip}_C\left(\nabla_{\bm{\theta}} \ell_i(\bm{\theta}_{k})\right) + \gauss \left(0, C^2 \sigma^2 \mathbf{I} \right) \right],}
\end{equation}
where $\ell_i(\bm{\theta})$ is the  per-sample loss function evaluated at sample $\mathbf{x}_i$. 
We also use the term ``DP-SGD'' loosely to refer to the category of gradient-based optimization algorithms that operate on the noisy gradient, \emph{e.g.}, Adam~\citep{kingma2014adam}.
The privacy analysis of DP-SGD relies on composition of multiple steps.
One particularly powerful analysis framework amenable to such compositions relies on a variant of DP called R\'{e}nyi differential privacy (RDP) \citep{mironov2017renyi}.
An advantage of RDP is its additive composition property, where the privacy guarantees of a sequence of mechanisms can be combined with amplification by subsampling~\citep{wang2019subsampled} and then translated to $(\varepsilon, \delta)$-DP~\citep{balle2020hypothesis, gopi2021numerical}. 
In this work, we adopt this accounting technique.

























\textbf{Scaling up DP-SGD training.} DP training is a theoretically and empirically proven remedy against unintended training data memorization.
Even models with large $\varepsilon$ (\emph{e.g.}, $\varepsilon=100$) can empirically defend against privacy attacks~\citep{carlini2021membership, guo2023analyzing}. 
Despite its great appeal, DP training also carries a significant drawback of large drop in model utility~\citep{abadi2016deep,tramer2020differentially}.
For example, the SOTA performance on ImageNet when training from scratch with a DP guarantee of $\varepsilon=8$ is 39.2\%~\citep{sander2023tan}; in comparison, the non-private performance on ImageNet when training from scratch can reach 88\%~\citep{touvron2022deit} or higher. This degradation in model utility also translates to poorly learned representations, as \citet{tramer2020differentially} showed that even handcrafted features can rival ones learned through DP training.


\citet{yu2023vip} made the first step towards obtaining high-utility learned representations through scaling DP training. They proposed self-supervised learning (SSL) on internet-scale data as a solution for the privacy-utility trade-off in DP representation learning.
Among the numerous SSL algorithms, the authors observed that the reconstruction-based approach of masked autoencoder (MAE; \citet{he2022masked}) is compatible with the requirements of DP-SGD.
By leveraging weight initialization through synthetic pre-training, the authors were able to obtain high-utility learned representations at a strict privacy budget of $\varepsilon=8$. 
Compared to ViP~\citep{yu2023vip}, we demonstrate that the image captioning approach (see Section ~\ref{subsec:pretrain-captioners-with-DPSGD}) learns much better image representations by utilizing the additional text supervision. 














==> Untitled/3-method.tex <==
\vspace{-0.05in}
\section{Approach
}\label{sec:approach}




We describe in detail our approach of DP representation learning via image captioning. We first argue why image captioning is intuitively a suitable objective for obtaining better image representations via DP-SGD training (section \ref{subsec:pretrain-captioners-with-DPSGD}). Then, we elucidate the technical challenges that we resolved to make DP training viable and effective for image captioning (section \ref{subsec:effective_strategies_DPCAP}).

\vspace{-0.02in}
\subsection{DP Representation Learning via Image Captioning}\label{subsec:pretrain-captioners-with-DPSGD}



\textbf{Why is vision-language pre-training suitable?} %
Given image-text aligned datasets, prior works~\citep{radford2021learning, li2022blip, tschannen2023image} showed that pre-training using language supervision is an appealing option for non-private representation learning. We hypothesize that this is true for DP representation learning as well. Compared to image-only supervision, language supervision contains a more condensed summary of the image content, allowing the model to ignore irrelevant details such as background and focus on objects of interest and their relationships. 
This is especially helpful for DP since the model needs to extract as much useful information as possible from each sample given the privacy budget $\varepsilon$.
Captioning could thus enhance the privacy-utility-sample size trade-off in DP, considering it requires less information per sample.

In addition, we show that vision-language pre-training supports a very large batch size, much larger than what is typically used in image-only pre-training~\citep{radford2021learning, li2022blip, yu2022coca}. 
This subtle aspect is in fact crucial for reducing the effective noise in DP-SGD~\citep{li2021large}, which allows the model parameters to converge to a stable solution with lower training loss (see Section~\ref{subsec:effective_strategies_DPCAP}). 



\textbf{Vision-language pre-training via image captioning.} 
Perhaps the most popular approach for vision-language pre-training is contrastive language image pre-training (CLIP; \citet{radford2021learning}) as well as its variants~\citep{mu2022slip, li2023scaling}.   
However, the contrastive loss used in these methods is not an additive function over the samples, \emph{i.e.}, it cannot be written in the form $\sum_{i} \ell_i$, where $\ell_i$ depends only on the $i$-th sample.
Thus, DP-SGD~(\emph{cf.} \eqref{eq:DP_SGD}) cannot be directly applied.

Unlike contrastive learning, the image captioning approach~\citep{sariyildiz2020learning,desai2021virtex, tschannen2023image} aligns well with DP-SGD training.
Specifically, an image captioner is trained to predict captions based on their corresponding images. 
The training objective of the image captioner for one image-text pair $[\mathbf{x}^{\text{img}}, \mathbf{z}^{\text{text}}]$ is to minimize over $\bm{\theta}:=\{\bm{\theta}_{\textsf{enc}}, \bm{\theta}_{\textsf{dec}}\}$ the following loss:
\vspace{-0.1in}
\revisioncolor{
\begin{align}\label{eq:loss-image-captioner}
 &L_{\text{Cap}}(\bm{\theta}) 
 := \frac{1}{T}\sum_{t=0}^{T-1} \ell_{\text{CE}}\Big({z}^{\text{text}}_{t+1}, \varphi\big(\mathbf{z}^{\mathrm{img}}, \mathbf{z}_{1:t}^{\mathrm{text}}; \bm{\theta}_{\textsf{dec}}\big)\Big), \\
 &\mathrm{where}\, \mathbf{z}^{\mathrm{img}}=\underbrace{\psi(\mathbf{x}^{\text{img}}; \bm{\theta}_{\textsf{enc}})}_{\text{image embedding}}, \,\, \mathbf{z}^{\mathrm{text}}_{1:t} = \underbrace{{z}^{\text{text}}_1,
\ldots, {z}^{\text{text}}_{t}}_{\text{first $t$ tokens}}. \nonumber 
\vspace{-0.2in}
\end{align}
}

\vspace{-0.1in}
\noindent
We use $\mathbf{z}^{\text{text}}$ denotes the caption token sequence $ \{{z}^{\text{text}}_1,
\ldots, {z}^{\text{text}}_{T}\}$, \revisioncolor{ and we let $\bm{z}_{1:0}^{\mathrm{text}} = \emptyset$.} 
The image captioner consists of two parts: the image encoder $\psi(\cdot; \bm{\theta}_{\textsf{enc}})$ and the text decoder $\varphi(\cdot; \bm{\theta}_{\textsf{dec}})$. 
The rationale behind the design of \eqref{eq:loss-image-captioner} is that the image encoder maps the input image $\mathbf{x}^{\text{img}}$ to an embedding vector, and the text decoder takes the image embedding $\psi(\mathbf{x}^{\text{img}}; \bm{\theta}_{\textsf{enc}})$ and the first $t$ caption tokens $\{{z}^{\text{text}}_1,
\ldots, {z}^{\text{text}}_{t}\}$ as inputs and predicts the next caption token ${z}_{t+1}^{\text{text}}$.
Both the encoder and decoder are trained to maximize the log-likelihood of the correct next token. 
Equation~\ref{eq:loss-image-captioner} corresponds to the loss function for an image-text pair $[\mathbf{x}^{\text{img}}, \mathbf{z}^{\text{text}}]$; summing over all the samples in a batch gives the complete empirical loss in an additive form, which is directly compatible with DP-SGD.

\revisioncolor{
\textbf{Interpretation of DP bound for image-text pairs.} $\varepsilon$-DP bounds the amount of information extracted from each training sample by $\varepsilon$. For DP-Cap, each sample is made of \{image + caption\}, while ViP~\cite{yu2023vip} utilizes \{image\} only. Consequently, DP-Cap inherently offers an equivalent or better privacy guarantee for each image. 
To better understand this, we can consider membership inference attacks~\citep{shokri2017membership} as an example.
Suppose $\varepsilon$-DP upper bounds the success rate of the membership inference attack (when given the image-text pair) against DP-Cap as less or equal to $p$. 
Then the MIA success rate when given only the image can be at most $p$ since the attacker has strictly less information. 
This is exactly the upper bound for the success rate of a membership inference attack against ViP. }


\vspace{-0.2cm}
\subsection{Strategy for Effective DP Training}\label{subsec:effective_strategies_DPCAP}



\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figs/fig3_vision_yy.pdf}
  \vspace{-0.25in}
  \caption{Impact of synthetic initialization on DP-Cap. 
  The learned image representation benefits substantially from initializing on the Shaders21K dataset. The
  gap between DP-Cap (random init) and DP-Cap (syn init) can be as large as 24\% when evaluated using linear probing on ImageNet.}
  \vspace{-0.25in}
  \label{fig:benefit-syn-pretrain}
\end{figure}


Although image captioning has demonstrated impressive representation learning capabilities in the non-private regime, adapting it to DP training requires careful considerations.
To obtain a useful pre-trained model, one needs to train for a sufficient number of steps under a low effective noise, both of which are at odds with obtaining a strong privacy guarantee.
We detail the strategy we used to handle this trade-off when training the image captioner. 

\begin{figure*}[t!]
  \centering
  \begin{subfigure}{0.49\textwidth}
  \centering
    \includegraphics[width=\linewidth]{figs/figure2_CP_new.pdf}
    \caption{DP-Cap scales gracefully to extreme batch sizes}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth} 
  \centering
  \includegraphics[width=0.95\linewidth]{figs/fig3a_test_mae.pdf}
    \caption{Performance improves consistently with larger batch size}
  \end{subfigure}
  \vspace{-0.05in}
  \caption{(a) We fix the effective noise $\sigma/B = 5.6 \times 10^{-7}$ \blue{(corresponding to our (B, $\sigma$) = (1.3M, 0.728))} and show that the loss is remarkably consistent across different batch sizes, allowing us to effectively scale up batch size to improve the SNR. (b) Performance from 4 sets of parameters that provide $\varepsilon=8$, with constant number of steps 5708. From batch size 98k (used in ViP~\citep{yu2023vip}), to our 1.3M batch size.
  In contrast to ViP, DP-Cap successfully leverages the better SNR and learns features that achieve substantially better 10-shot accuracy on ImageNet even compared to a \textbf{non-private} MAE \citep{he2022masked} trained on the same dataset (see Appendix~\ref{sec:appendix_optim}).}
  \label{fig:3}
  \vspace{-2ex}
\end{figure*}



\textbf{Sufficient number of training steps.} 
We address this challenge via synthetic pre-training. 
Image representations learned by \textit{DP-Cap (random init)}  outperform those of \textit{ViP (random init)} as evidenced in table~\ref{tab:appendix_randominit} in Appendix~\ref{sec:appendix-additional-exp-results}. 
Interestingly, ~\citet{yu2023vip} \revisioncolor{and ~\citet{tang2024differentially} have shown that synthetic images consisting of only textures can provide a good initialization for training DP models without any privacy risk. 
With this initialization in ~\citet{yu2023vip}, the reconstruction-based model }can \revisioncolor{then} focus on learning dataset-specific properties rather than low-level image properties such as edge detectors, therefore expending privacy budget in a more optimal manner.
We adapt this technique of pre-training on the Shaders21K dataset~\citep{baradad2022procedural} for initialization and observe that it is even more effective with DP-Cap compared to ViP.\footnote{\revisioncolor{For the synthetic pre-training on Shders21k in DP-Cap, we modify the training of image captioning model such that the model is trained to predict missing image patches, which is similar to MAE~\cite{he2022masked}. More details can be found in Appendix~\ref{sec:appendix_optim}.  }}
As shown in Fig.~\ref{fig:benefit-syn-pretrain}, our \textit{DP-Cap (syn init)} improves over \textit{DP-Cap (random init)} by more than 24\% on ImageNet-1k linear probing. It also improves over synthetic initialization alone (\textit{Syn-init}) by more than 14\% on ImageNet-1k linear probing, whereas the gain in ViP is smaller than 6\%. 





\textbf{Using extreme batch sizes to reduce effective noise.} \citet{li2021large} first showed that increasing the batch size in DP-SGD often improves the privacy-utility trade-off. This is because the effective noise added to the average gradient has magnitude $\sigma / B$ (\emph{cf.} \eqref{eq:DP_SGD}), and that increasing $B$, rather than decreasing $\sigma$, results in better privacy guarantees according to conventional accounting techniques~\citep{bun2016concentrated, dwork2016concentrated, mironov2019r, sander2023tan}.
\revisioncolor{However, in supervised learning, increasing the batch size beyond a certain point may degrade performance in both private and non-private settings~\citep{sander2024implicit}}.
Specifically,~\citet{sander2023tan} 
observed that when training a classifier from scratch with DP-SGD on ImageNet, at a fixed number of steps $S$ and fixed effective noise $\sigma/B$, the performance decreases significantly when the batch size becomes too large: for $B \in [128, 16384]$, a drop of 10\% in top-1 accuracy was observed.








Intriguingly, we find that vision-language pre-training on internet-scale datasets can tolerate \emph{extreme} batch sizes, \emph{e.g.} $B=1$M.
In Figure~\ref{fig:3}(a), we compare the loss behaviors when scaling the batch size for DP-Cap. We fix the effective noise $\sigma/B$ while varying the batch size.
In stark contrast to the previous observation from \cite{sander2023tan}, the loss trajectory is identical across different batch sizes. 
With this observation, we are able to successfully scale up the batch size for DP-Cap to as large as $B=1.3$M, achieving an effective noise of $5.6\times10^{-7}$, almost 10 times smaller than the effective noise of ViP in \citet{yu2023vip}.
Training DP-Cap under such a small effective noise allows it to extract information from the training dataset more efficiently under the DP constraint. 
In Figure~\ref{fig:3}, we show that with $B=1.3$M, the representation learned by DP-Cap even outperforms \emph{non-private} MAE trained on the same dataset. 
\revisioncolor{From these results, we find that the DP-Cap training can handle extreme large batches much more effectively than ViP in the context of differentially private training. This advantage is likely independent of image captioning models's inherent superiority over MAE. }




\begin{figure*}[t!]
    \begin{minipage}[c]{0.52\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/compute_cost_v2.pdf}
        \vspace{-5ex}
        \caption{Number of GPU hours to train DP-Cap for a single epoch on 233M samples. For the Large model, we achieve a close to $5\times$ reduction.\label{fig:compute_cost}}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|cccc}
    	\toprule
    	\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Model}} \\
            & Tiny & Small & Base & Large \\
            \midrule
    	\midrule
            \texttt{functorch} &  36 & 20 & 12 & 5 \\
            \cmidrule(lr){1-5} 
    	Ghost norm & 350 & 230 & 180 & 64 \\
            \cmidrule(lr){1-5} 
    	  Ghost norm+AMP & 420 & 310 & 225 & 90 \\
    	\bottomrule
        \end{tabular}
        }
        \captionof{table}{Max physical batch size under different per-sample gradient computation methods.\label{tab:max_batchsize}}
    \end{minipage}
    \vspace{-2ex}
\end{figure*}

\textbf{Improving training pipeline efficiency.} DP training is known to be computationally inefficient due to factors such as per-sample gradient computation~\citep{lee2020scaling, li2021large}. 
Training on internet-scale datasets using extreme batch sizes further complicates this issue. 
For example, a naive implementation of DP-Cap with per-sample gradient computation using \texttt{functorch} would take approximately 61 days(!) on 128 NVIDIA V100 GPUs. 
\revisioncolor{Recent studies~\citep{li2021large, bu2023differentially} have enhanced this efficacy by enabling DP training without the necessity to store per-sample gradients.}
We made significant efficiency improvements to the training pipeline using two techniques: ghost norm~\citep{li2021large} and the automatic mixed precision (AMP) package in PyTorch. 
Combining these two techniques with DP-SGD requires careful considerations to ensure both a correct DP guarantee as well as numerical stability. 
We detail the implementation in Appendix~\ref{app:computation}.

In Figure \ref{fig:compute_cost} we compare the compute cost of different gradient computation methods: \texttt{functorch}, ghost norm and ghost norm+AMP. The number of GPU hours is estimated on a single NVIDIA V100 GPU with 32GB memory using 100K samples. 
The improvement is especially notable for our largest model: Using ghost norm+AMP, we achieve a $4.7\times$ speedup compared to \texttt{functorch} and $3.3\times$ speedup compared to ghost norm alone, which amounts to a reduction from 61 days to 13 days when training for 32 epochs---a large but manageable compute cost. 
This improvement is due to both a more efficient forward-backward pass, as well as enabling a larger physical batch size; see Table \ref{tab:max_batchsize}. 
In addition, we adopt the TAN simulation framework~\citep{sander2023tan} to reduce the compute cost during hyperparameter search. 
Due to the batch size scaling behavior depicted in Figure \ref{fig:3}, TAN simulation is ideal for DP-Cap training and allows for rapid experimentation to identify promising methods before launching a full training run.






















































































==> Untitled/4-experiments.tex <==
\section{Evaluation}\label{sec:evaluation}


We demonstrate the representation learning capabilities of DP-Cap on both vision ({\small\textsf{V}}) and vision-language ({\small\textsf{V-L}}) downstream tasks. For all evaluations, the DP-Cap model is first pre-trained using DP-SGD on a subset of LAION-2B~\citep{Schuhmann2022LAION5BAO}, and then fine-tuned non-privately on a downstream dataset.

\subsection{Downstream Tasks}\label{subsec:tasks}

\textbf{Linear probing ({\small\textsf{V}}).} We train a linear classifier on top of learned representations and evaluate its accuracy. We consider both full linear probing using the full downstream dataset, as well as few-shot linear probing, which subsamples the downstream dataset down to $K$ samples per class. Few-shot linear probing is especially useful for evaluating learned representations since the model must rely heavily on the generalizability of representations in order to perform well under data scarcity.

\textbf{Zero-shot image classification ({\small\textsf{V-L}})} is one of the most widely used methodologies for evaluating vision-language models~\citep{radford2021learning}. 
A strong zero-shot performance suggests that the image representation aligns well to text.
We perform zero-shot classification using the DP-Cap image encoder and text decoder by evaluating the likelihood of captions of the form ``this is a photo of a [label]''. We enumerate over different labels and predict the class that has the highest likelihood; see Section~\ref{sec:appendix_zero_shot} for full details.

\textbf{ARO (Attribution, Relation, and Order) ({\small\textsf{V-L}}).} The ARO benchmark~\citep{yuksekgonul2022and} can be used to gauge the adeptness of VLMs in understanding the compositional relationship between objects and attributes. A strong performance on ARO suggests that the learned image representation encodes semantic relationships such as ``the horse is eating the grass'' vs. ``the grass is eating the horse''.

\subsection{Experimental Setup}\label{subsec:exp-setup}
We present an overview of the experimental setup; refer to Appendix~\ref{sec:appendix-additional-details} for additional details.


\begin{table*}[t!]
	\centering
	\caption{Linear probing evaluation on downstream classification. Results for DP-NFNet, TAN, AlexNet and SimCLR are obtained from \citet{yu2023vip}. 
    For ViP \citep{yu2023vip}, we train with the same privacy parameters as for DP-Cap on the deduplicated dataset. More details are given in Appendix~\ref{sec:appendix_optim}.}
	\vspace{-0.05em}
	\resizebox{0.9\textwidth}{!}{
	    \footnotesize
		\begin{tabular}{llc|cccc}
			\toprule
			\multirow{1}{*}{Model} &   \multirow{1}{*}{pretraining data}  & \multirow{1}{*}{ DP? } 
			&   \multirow{1}{*}{ ImageNet-1K  } & \multirow{1}{*}{ Places-365 } & \multirow{1}{*}{ Places-205 } &  \multirow{1}{*}{iNat-2021}  
			  \\
            \midrule
		\midrule
		DP-NFNet  & ImageNet-1K &   {\large \textcolor{ao}{\ding{51}}}      &  45.3\%  &   40.1\% &  39.2\% &  28.2\% 
			\\ 
        \cmidrule(lr){1-7} 
		TAN   & ImageNet-1K & {\large \textcolor{ao}{\ding{51}}}    &   49.0\%  &  40.5\%  & 38.2\%  & 31.7\% 
			\\ 
        \cmidrule(lr){1-7} 
        {\color{gray} AlexNet }  & ImageNet-1K&{\large \textcolor{upsdellred}{\ding{55}}}  &   {\color{gray} 56.5\%}  &  {\color{gray} 39.8\%}  &  {\color{gray} 35.1\%} & {\color{gray} 23.7\%} 
			\\ 
        \cmidrule(lr){1-7} 
        {\color{gray} SimCLR }   & ImageNet-1K&{\large \textcolor{upsdellred}{\ding{55}}}  &  {\color{gray} 67.5\%}  & {\color{gray} 46.8\%}   & {\color{gray} 49.3\%}  & {\color{gray} 34.8\%}  
			\\ 
        \cmidrule(lr){1-7} 
		  {\color{gray} Cap} &  Dedup-LAION-233M &{\large \textcolor{upsdellred}{\ding{55}}} &  {\color{gray} 77.5\%} &  {\color{gray} 56.3\%} &  {\color{gray} 63.9\%}  &   {\color{gray} 63.9\%}
			\\ 
        \cmidrule(lr){1-7} 
		  {\color{gray} MAE} &  Dedup-LAION-233M &{\large \textcolor{upsdellred}{\ding{55}}} &  {\color{gray} 62.5\%} &  {\color{gray} 51.0\%} &  {\color{gray} 54.7\%}  &   {\color{gray} 42.3\%}
			\\ 
        \midrule
        \midrule
        {ViP}   & Dedup-LAION-233M &{\large \textcolor{ao}{\ding{51}}}   &  {56.5\%}  & {47.7\%}   & {49.6\%}  & {38.2\%}  
			\\ 
        \cmidrule(lr){1-7} 
        \cmidrule(lr){1-7} 

		  DP-Cap &  Dedup-LAION-233M & {\large \textcolor{ao}{\ding{51}}}  & {63.4\%} & {51.9\%}&  {54.3\%} & {44.5\%}
			\\ 
			\bottomrule
		\end{tabular}
	}
	\label{tab:main-table-linearprobing}
	\vspace{-0.2em}
\end{table*}

\begin{table*}[t!]
	\centering
	\caption{Performance of DP-Cap on zero-shot classification and compositional understanding (ARO). CLIP's zero-shot results are obtained from \citet{radford2021learning} (base model). For ARO, see Appendix~\ref{sec:appendix_ARO}.
 }
	\vspace{-0.1em}
	\resizebox{0.9\textwidth}{!}{
	    \footnotesize
		\begin{tabular}{lc|ccc|cccc}
			\toprule
			\multirow{2}{*}{Model}  & \multirow{2}{*}{ DP? } 
			& \multicolumn{3}{c|}{Zero-shot} 
			   & \multicolumn{4}{c}{ARO} 
			  \\[0.05em]
		  &  & ImageNet-1k  & CIFAR10 &  CIFAR100  & VGR  & VGA & COCO & Flickr 
			\\ 
            \midrule
        \midrule
    {Random Chance} & {-} & 0.1\%  &  10\% & 1\% & 50\% & 50\% & 20\% & 20\% 
			\\ 
        \midrule
    {\color{gray} CLIP } & {\large \textcolor{upsdellred}{\ding{55}}} &   {\color{gray}62.2\%} &  {\color{gray}91.3\%} &  {\color{gray}65.1\% }
    &  {\color{gray}62.4\%} &  {\color{gray}62.9\%} &  {\color{gray}47.8\%} &  {\color{gray}58.0\%}
			\\ 
    {\color{gray} Cap } & 
    {\large \textcolor{upsdellred}{\ding{55}}} &  {\color{gray}25.2\%}  &  {\color{gray}90.0\%}&  {\color{gray}37.4\%} &  {\color{gray}59.9\%} &  {\color{gray}87.2\%} &  {\color{gray}87.0\%} &  {\color{gray}87.4\%} 
			\\ 
    \midrule
    \midrule
    DP-Cap & {\large \textcolor{ao}{\ding{51}}} &  {7.8\%} & {54.4\%} & {16.4\%}  & {58.6\%} & {82.4\%} & {86.6\%}  & {87.2\%} 
			\\ 
			\bottomrule
		\end{tabular}
	}
	\label{tab:main-table-ARO}
	\vspace{-0.75em}
\end{table*}


\textbf{Datasets.} 
Following the approach introduced by \citet{yu2023vip}, we first pre-train on the Shader21k dataset~\citep{baradad2022procedural} of synthetic images.
We then train with DP-SGD on a subset comprising 233 million deduplicated (using SemDeDup~\citep{abbas2023semdedup}), NSFW-filtered and face-blurred (using an approach similar to \citet{yang2021obfuscation}) image-caption pairs from the (English-only) LAION-2B dataset~\citep{Schuhmann2022LAION5BAO}. We refer to this dataset as Dedup-LAION-233M.

We use the ImageNet-1K~\citep{Imagenet,Imagenet2}, CIFAR-10/100~\citep{krizhevsky2009learning}, Places-365/205~\citep{zhou2014learning} and iNaturalist-2021~\citep{van2021benchmarking} image classification datasets to assess the performance of learned image representations via full linear probing, few-shot linear probing, and zero-shot prediction. 
For vision-language tasks, we employ the Visual Genome Attribution (VGA), Visual Genome Relation (VGR), COCO-order~\citep{lin2015microsoft} and Flickr-30k~\citep{plummer2016flickr30k} datasets from the ARO benchmark~\citep{yuksekgonul2022and}. %
Finally, we evaluate image captioning using the MS-COCO 2017~\citep{lin2015microsoft} test set; result is shown in Figure~\ref{fig:1}(c) and Appendix~\ref{subsec:appendix-image-caption}.


\textbf{Model and training.} We use a transformer architecture~\citep{vaswani2017attention} for both the encoder and the decoder of DP-Cap, where the decoder applies causal cross-attention. 
\revisioncolor{We train DP-Cap model from scratch, including the embedding layer, with vocabulary size around 32,000.}
See Section~\ref{sec:appendix_optim} and \citet{tschannen2023image} for details. 
For privacy accounting we use R\'{e}nyi DP composition along with privacy amplification via Poisson subsampling~\citep{mironov2019r}, and convert to DP using \citet{balle2020hypothesis} through the Opacus library~\citep{yousefpour2021opacus}, targeting $\delta=1/N$ where $N$ represents the number of training samples. We refer to the non-private counterpart of DP-Cap trained on the same dataset as ``Cap''.

\subsection{Main Results}\label{subsec:eval-v-and-vl}



\begin{table*}[t!]
	\centering
	\caption{Ablation studies on the effect of dataset size and privacy budget $\varepsilon$ on DP-Cap (base). 
 }
	\vspace{-0.3em}
	\resizebox{\textwidth}{!}{
	    \footnotesize
		\begin{tabular}{llccc|cccc|cccc}
			\toprule
            \multirow{1}{*}{$\varepsilon$}
			& 
            \multirow{1}{*}{$\sigma$} & 
            \multirow{1}{*}{\# Data} &   
            \multirow{1}{*}{\# Steps} & 
            \multirow{1}{*}{$B$} 
			&   \multicolumn{4}{c|}{ImageNet-1K}   & \multicolumn{4}{c}{ARO ({\small\textsf{V-L}})}  
			  \\
            \midrule
		\midrule
		{ } & { } & { }   &  { } &  { }  & {0-shot} ({\small\textsf{V-L}})  & {1-shot} ({\small\textsf{V}}) &  {2-shot} ({\small\textsf{V}}) & {10-shot} ({\small\textsf{V}}) & {VGR} & {VGA} & {COCO} & {Flickr} 
			\\ 
  \midrule[\heavyrulewidth] 
		{\color{gray} $+\infty$} &
  {\color{gray} 0} &{\color{gray} 233M}   &  {\color{gray} 60,000}  &  {\color{gray} 40,960}     & {\color{gray}  {25.2\%} } &  {\color{gray} {27.0\%}} & {\color{gray} {37.2\%}} & {\color{gray} {57.9\%}} & {\color{gray} {59.9\%}} & {\color{gray} {87.2\%}} & {\color{gray} {87.0\%}}  & {\color{gray} {87.4\%}} 
			\\ 

        \cmidrule(lr){1-13} 
		 {8.0} & {0.728} &{233M} & {5708}  &  {1.3M}  &  
   \blue{7.8\%}    & \blue{10.3\%} &  \blue{15.6\%} & \blue{31.8\%} & \blue{58.6\%} & \blue{82.4\%} & \blue{86.6\%}
        & \blue{87.2\%} 
			\\ 

        \cmidrule(lr){1-13} 
		 {2.0} & {1.18} &{233M} & {2854} &  {1.3M}  &  \blue{3.2\% }    & \blue{7.0\%} &  \blue{10.8\%} & \blue{23.9\%} & \blue{58.5\% } & \blue{79.7\%} & \blue{85.3\% } & \blue{86.6\%} 
			\\ 

        \cmidrule(lr){1-13}  
		 {1.0} & {1.5} & {233M} &  {1427} &  {1.3M}  
   &  \blue{1.1\%}    & \blue{5.2\%} &  \blue{8.2\%} & \blue{19.9\%} & \blue{58.3\%} & \blue{75.6\%} & \blue{83.9\%} & \blue{85.3\%} 
			\\ 
        \cmidrule(lr){1-13} 
         8.0 & {0.728} & 23M  & {5708}&  {130K}   
        &  \blue{0.7\%}
        &  \blue{3.4\%}
        &  \blue{5.3\%}
        & \blue{13.3\%}  
        &  \blue{58.3\%}
        &  \blue{76.2\%}
        &  \blue{84.9\%}
        &  \blue{85.9\%} 
			\\ 
        \cmidrule(lr){1-13} 
         8.0 & {0.728} & 2.3M & 5708 &  {13K}  
        & \blue{0.1\%}    
        & \blue{1.8\%}
        & \blue{2.9\%}
        & \blue{8.1\%}
        & \blue{57.6\%}
        & \blue{66.4\%}
        & \blue{79.5\%}
        & \blue{82.0\%}
			\\ 
			\bottomrule
		\end{tabular}
	}
	\label{tab:eps-datasize}
	\vspace{-0.4em}
\end{table*}

\begin{table*}[t!]
	\centering
	\caption{Ablation studies on the effect of model size.
  We compare ViP and DP-Cap's number of encoder parameters. More details about the DP-Cap models can be found in Table~\ref{tab:appendix-table-cap-model-size}.
} %
	\vspace{-0.5em}
	\resizebox{\textwidth}{!}{
	    \footnotesize
		\begin{tabular}{llc|ccccc|cccc}
			\toprule
			\multirow{1}{*}{Model} & \multirow{1}{*}{Config} & 
            \multirow{1}{*}{\# parameters}  
			&  \multicolumn{5}{c|}{ImageNet-1K (Vision)}   & \multicolumn{4}{c}{ARO (Vision-Language)} 
			  \\
            \midrule
		\midrule
		{ } &   { }     & { }     & {1-shot} &  {2-shot} & {5-shot} & {10-shot} & \blue{LP} & {VGR} & {VGA} & {COCO} & {Flickr}
			\\ 
        \midrule[\heavyrulewidth] 
        {ViP} & Base &  86.6M  &  2.5\%    
        &  4.2\%
        & 8.5\%
        &  14.3\% 
        & \blue{56.5\%}
        & /  
        & /
        & /
        & /
			\\ 
        \midrule
		{DP-Cap}  & Tiny &  22.0M
        & \blue{7.9\%} 
        & \blue{12.1\%}
        & \blue{18.7\%}
        & \blue{25.2\%}
        & \blue{57.5\%}
        & \blue{58.6\%}
        & \blue{79.1\%}
        & \blue{85.7\%}
        & \blue{87.1\%}
			\\ 
        \cmidrule(lr){1-12} 
		{DP-Cap}  & Small &  49.0M
        & \blue{9.0\%} 
        & \blue{14.0\%}  
        & \blue{21.6\%}
        & \blue{28.9\%}
        & \blue{61.1\%}
        & \blue{59.1\%}
        & \blue{80.5\%}
        & \blue{86.0\%}
        & \blue{86.6\%}
			\\ 
        \cmidrule(lr){1-12} 
		{DP-Cap}  & Base &  86.6M
        & \blue{10.3\%}
        &  \blue{15.6\%}  
        & \blue{24.2\%}
        & \blue{31.8\%}  
        & \blue{63.4\%}
        &\blue{58.6\%}& \blue{82.4\%}& \blue{86.6\%}
        & \blue{87.2\%} 
			\\ 
        \cmidrule(lr){1-12} 
		{\blue{DP-Cap}}  & \blue{Large} &  \blue{407.3M}
        & \blue{11.8\%}
        &  \blue{17.5\%}  
        & \blue{26.2\%}
        & \blue{34.0\%}  
        & \blue{65.8\%}
        &\blue{59.5\%}& \blue{80.1\%}& \blue{86.6\%}
        & \blue{86.5\%} 
			\\ 
			\bottomrule
		\end{tabular}
	}
	\label{tab:scaling-model-size}
	\vspace{-0.4em}
\end{table*}


\textbf{Linear probing evaluation ({\small\textsf{V}}).} 
We assess the performance of the vision encoder on downstream tasks via linear probing.
In Fig~\ref{fig:1}(a), we compare the performance of DP-Cap and ViP \citep{yu2023vip} on ImageNet-1k few-shot linear probing. 
DP-Cap significantly improves over ViP, with up to $\times$2.5 better performance across different shots.
In addition, we evaluate the full linear probing accuracy of DP-Cap, ViP and other baselines in Table~\ref{tab:main-table-linearprobing}.
DP-Cap outperforms ViP and other DP models, including TAN~\citep{sander2023tan} and DP-NFNet~\citep{DeepMindUnlocking}, across all tasks.
DP-Cap even outperforms non-private AlexNet~\citep{krizhevsky2012imagenet} and except on ImageNet, SimCLR~\citep{simclr} (\blue{both were trained on ImageNet}).
We provide additional results for fine-tuning on downstream datasets in Table~\ref{tab:main-table-finetune-fewshot} (App.~\ref{sec:appendix-additional-exp-results}), also showing improvements over competing methods.







\textbf{Zero-shot performance ({\small\textsf{V-L}}).}
In the left three columns of Table~\ref{tab:main-table-ARO}, we evaluate the zero-shot performance of DP-Cap compared to non-private Cap and CLIP/BLIP on ImageNet-1k and CIFAR10/100.
Contrastive methods such as CLIP and BLIP have demonstrated greater suitability for zero-shot prediction compared to image captioning approaches~\citep{tschannen2023image}, which is evident by the disparity between the performance of Cap and CLIP/BLIP. 
Nevertheless, we observe that DP-Cap achieves noteworthy zero-shot classification performance that is significantly above random chance, and stands as the first DP model to do so. This accomplishment marks a promising milestone for DP training, although there remains a substantial performance gap between DP-Cap and Cap.


\textbf{Attribution, Relation, and Order (ARO) evaluation ({\small\textsf{V-L}}).} 
Contrastive-based methods such as CLIP often exhibit behavior akin to bag-of-words models~\citep{yuksekgonul2022and, tejankar2021fistful, basu2023augmenting}, making them less adept at performing well on the ARO benchmark. Remarkably, DP-Cap significantly outperforms \emph{non-private} CLIP in this context (see Fig~\ref{fig:1}(b) and Table~\ref{tab:main-table-ARO}), and even achieves performance close to that of \emph{non-private} Cap. Our result shows that DP training can be particularly effective for learning complex compositional relationships.



\vspace{-0.15cm}
\subsection{Ablation Studies}\label{subsec:dp-cap-scaling}

We perform ablation studies on the scaling behavior of DP-Cap with respect to the dataset size, privacy budget and model size. In Appendix~\ref{sec:appendix-additional-exp-results}, we show additional results on image captioning and on the impact of compute budget.

\textbf{Scaling dataset size.} We show that dataset scaling is crucial for effectively training DP-Cap as it results in better SNR under the same privacy budget (see Figure~\ref{fig:eps_N}).
We randomly subsample 1\% and 10\% of the Dedup-LAION-233M dataset, which is used for training our default DP-Cap-Base model in Table~\ref{tab:main-table-linearprobing} (denoted by Dedup-LAION-2M and Dedup-LAION-23M). 
We set the batch size to $B/100$ for Dedup-LAION-2M and $B/10$ for Dedup-LAION-23M, respectively. This allows the model to be trained for the same number of steps across the different datasets, although at a much larger effective noise level.
As shown in Table~\ref{tab:eps-datasize}, the number of training samples is critical for achieving strong performance for DP-Cap models: the zero-shot performance of our model trained on 1\% of the dataset achieves random zero-shot performance on ImageNet and much worse accuracy across the board on ARO.


\textbf{Impact of the privacy budget $\varepsilon$.}
We also investigate the performance of DP-Cap under lower privacy budgets ($\varepsilon=1$ and $\varepsilon=2$), employing the same batch size of 1.3 million. 
The outcomes of these experiments are presented in Table~\ref{tab:eps-datasize}. 
As anticipated, the utility of our model does exhibit a decline with decreasing $\varepsilon$. However, the performance degradation is relatively minor for the learned representation, with 10-shot ImageNet performance decreasing from 31.8\% ($\varepsilon=8$) to 19.9\% ($\varepsilon=1$).
More surprisingly, the performance impact on ARO is nearly negligible.
It is noteworthy that both models continue to outperform previous state-of-the-art DP models trained with $\varepsilon=8$ (see Figure~\ref{fig:1}). 
This phenomenon can be attributed to the relatively small effective noise resulting from the extreme batch size, which for $\varepsilon=1$ remains five times smaller than that used in \cite{yu2023vip}.


\textbf{Scaling model size.} 
Scaling up the model size is one of the most effective approaches for training better non-private foundation models~\citep{brown2020language, bommasani2021opportunities, touvron2023llama}. 
\revisioncolor{However, an intuitive understanding of DP-SGD~\footnote{This is because the added noise has $L_2$ norm $\approx \sigma C \sqrt{d} / B$, where $d$ is the number of model parameters, whereas the gradient norm is constrained to $C$ regardless of model size.} 
suggests that scaling up model size does not improve utility in DP training since more model parameters will lead to lower signal-to-noise ratio, especially when training large DP models from scratch}. 
\revisioncolor{Recent work~\citep{li2022does} demonstrates that during DP fine-tuning, gradients occupy a lower effective dimensional subspace, and larger networks can enhance the performance of DP-SGD.}
To test this hypothesis \revisioncolor{in pre-training}, we train DP-Cap with different model sizes (Tiny, Small, Base, Large) using the same hyperparameters and evaluate their performance in Table~\ref{tab:scaling-model-size},\ref{tab:zero-shot-model-size-table-appendix}; see Table~\ref{tab:appendix-table-cap-model-size} for details about different model sizes.
We observe consistent improvements when scaling up the model from {DP-Cap-Tiny} to {DP-Cap-Large}.
Our observation suggests that DP-Cap has strong model scaling behavior even with DP-SGD training.



==> Untitled/5-discussion.tex <==
\vspace{-0.2cm}
\section{Discussion and Future Work}\label{sec:discussion}

We demonstrated that DP representation learning via image captioning is viable. In particular, image captioning is an ideal objective that supports both per-sample loss and large batch training---two critical ingredients in DP-SGD. When applied to the Dedup-LAION-233M dataset, the trained model learns useful image representations for downstream tasks and exhibits strong multi-modal capabilities. 

Through our study we also identify three open problems in the general direction of DP pre-training of large-scale foundation models that are difficult to handle with existing techniques:

\begin{enumerate}[leftmargin=*]
\item Scaling up the batch size to extreme levels is crucial for reducing the effective noise and facilitating model convergence. Is there a fundamental reason why image captioning can support extremely large batch training?
When the model does not scale well with batch size, is it due to poor optimization or is it inherent to the model and/or task? Answers to these question can help identify other successful training recipes that further improve the quality of DP-learned representations.
\item
Scaling up the model size is typically beneficial in non-private representation learning, but can be ineffective in DP training due to a decrease in gradient SNR. 
While we have observed a performance improvement from Tiny to Large, we anticipate that deterioration could occur when scaling up to a much larger model size, especially when the signal-to-noise ratio (SNR) undergoes a certain threshold.
Does this threshold exist? Can this trade-off be resolved through parameter-efficient architectures?
\item
Contrastive learning offers unique advantages compared to other multi-modal learning objectives such as learning image and text representations that are semantically aligned, but is not compatible with standard DP-SGD training. What techniques can enable differentially private contrastive learning?
\end{enumerate}







==> Untitled/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\newcommand{\calM}{\mathcal{M}}
\newcommand{\gauss}{\mathcal{N}}


\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

